A Certified Universal Gathering Algorithm for Oblivious Mobile Robots

We present a new algorithm for the problem of universal gathering mobile oblivious robots (that is, starting from any initial configuration that is not bivalent, using any number of robots, the robots reach in a finite number of steps the same position, not known beforehand) without relying on a common chirality. We give very strong guaranties on the correctness of our algorithm by proving formally that it is correct, using the COQ proof assistant. To our knowledge, this is the first certified positive (and constructive) result in the context of oblivious mobile robots. It demonstrates both the effectiveness of the approach to obtain new algorithms that are truly generic, and its managability since the amount of developped code remains human readable.

==> exemple3phases.tex <==


% 1                 7
% 2    3         6  8
% -------------------

% cas général -> les non-extr vont au centre (phase 3)
% (actifs, qui tu veux mais au moins 3 et 6 et 7 [qui ne bouge pas])



% 1        6        7
% 2        3        8
% -------------------

% cas 3 piles, on va sur celle du milieu (phase 2)
% (actif 1)


%          1
%          6        7
% 2        3        8
% -------------------

% Ooooh une pile majoritaire...(phase 1)
% (actifs : qui tu veux, de toute façon on reste dans ce cas maintenant)






\tikzstyle{rond}=[circle=1pt,draw=black,line width=1pt]

\newcommand{\robot}[3]{\node (r) at (#1,#2) [draw,color=#3,fill,rond] {};}



\begin{slide}  
  \myheader[\hfill mise en œuvre]{Preuves d'impossibilité}

\rule{0cm}{1.078cm}

%  \begin{overlayarea}{\linewidth}{4cm}
  \begin{center}
    \begin{tikzpicture}[scale=1.6]
      \node(dummy) at (-2,-1.5) {};
      \node(dummy) at (+3,+3) {};
      \begin{scope}[>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{3}{0cm}{gentil}
        \robot{3}{0.2cm}{gentil}
        \robot{3}{0.4cm}{gentil}
        \robot{3}{0.6cm}{gentil}
        \robot{0}{0cm}{gentil}
        \robot{0}{.2cm}{gentil}
        \robot{0}{.4cm}{gentil}
        \robot{0}{.6cm}{gentil}
        \node(col11) at (0,0) {};
        \node(col12) at (0,1cm) {};
        \node(col21) at (3,0) {};
        \node(col22) at (3,1cm) {};
%        \node<2->[draw=red,inner sep=10pt,thick,ellipse,fit=(col11) (col12)] {};
      \end{scope}
      \node(eq) at (5.5,0) {\Huge$\equiv$};
      \begin{scope}[xshift=4cm,>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{0}{0cm}{gray}
        \robot{0}{.2cm}{gray}
        \robot{0}{.4cm}{gray}
        \robot{0}{.6cm}{gray}
        \robot{3}{0cm}{gray}
        \robot{3}{0.2cm}{gray}
        \robot{3}{0.4cm}{gray}
        \robot{3}{.6cm}{gray}
      \end{scope}
    \end{tikzpicture}
  \end{center}
%\end{overlayarea}
%\begin{overlayarea}{1\linewidth}{1cm}
%    {~}
%  \end{overlayarea}

\vfill
\end{slide}

\begin{slide}  
  \myheader[\hfill mise en œuvre]{Preuves d'impossibilité}

\vfill

%  \begin{overlayarea}{\linewidth}{4cm}
  \begin{center}
    \begin{tikzpicture}[scale=1.6]
      \node(dummy) at (-2,-1.5) {};
      \node(dummy) at (+3,+3) {};
      \begin{scope}[>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{3}{0cm}{gentil}
        \robot{3}{0.2cm}{gentil}
        \robot{3}{0.4cm}{gentil}
        \robot{3}{0.6cm}{gentil}
        \robot{0}{0cm}{gentil}
        \robot{0}{.2cm}{gentil}
        \robot{0}{.4cm}{gentil}
        \robot{0}{.6cm}{gentil}
        \node(col11) at (0,0) {};
        \node(col12) at (0,1cm) {};
        \node(col21) at (3,0) {};
        \node(col22) at (3,1cm) {};
        \draw[->,color=red,inner sep=2pt,line width=3pt] (col12) 
        to [out=50,in=130] node [above] {\emphr{?}} (col22) ;
      \end{scope}
      \node(eq) at (5.5,0) {\Huge$\equiv$};
      \begin{scope}[xshift=4cm,>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{0}{0cm}{gray}
        \robot{0}{.2cm}{gray}
        \robot{0}{.4cm}{gray}
        \robot{0}{.6cm}{gray}
        \robot{3}{0cm}{gray}
        \robot{3}{0.2cm}{gray}
        \robot{3}{0.4cm}{gray}
        \robot{3}{.6cm}{gray}
      \end{scope}
    \end{tikzpicture}
  \end{center}
%\end{overlayarea}
%\begin{overlayarea}{1\linewidth}{1cm}
%    {~}
%  \end{overlayarea}

\vfill
\end{slide}

\begin{slide}  
  \myheader[\hfill mise en œuvre]{Preuves d'impossibilité}

\vfill

%  \begin{overlayarea}{\linewidth}{4cm}
  \begin{center}
    \begin{tikzpicture}[scale=1.6]
      \node(dummy) at (-2,-1.5) {};
      \node(dummy) at (+3,+3) {};
      \begin{scope}[>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{3}{0cm}{gentil}
        \robot{3}{0.2cm}{gentil}
        \robot{3}{0.4cm}{gentil}
        \robot{3}{0.6cm}{gentil}
        \robot{0}{0cm}{gentil}
        \robot{0}{.2cm}{gentil}
        \robot{0}{.4cm}{gentil}
        \robot{0}{.6cm}{gentil}
        \node(col32) at (0,1.63cm) {\rule{0pt}{2pt}};
        \node(col11) at (0,0) {};
        \node(col12) at (0,1cm) {};
        \node(col21) at (3,0) {};
        \node(col22) at (3,1cm) {};
        \node(col13) at (0,-0.7) {};
        \node(col23) at (3,-0.7) {};
        \draw[->,color=gentil,inner sep=2pt,line width=3pt] (col23) 
        to [out=-130,in=-50] (col13) ;
        \draw[->,color=gentil,inner sep=2pt,line width=3pt] (col12) 
        to [out=50,in=130] (col22) ;
        \node[draw=red,inner sep=10pt,thick,ellipse,fit=(col11)
        (col12)] {};
        \node[draw=red,inner sep=10pt,thick,ellipse,fit=(col21)
        (col22)] {};

      \end{scope}
      \node(eq) at (5.5,0) {\Huge$\equiv$};
      \begin{scope}[xshift=4cm,>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{0}{0cm}{gray}
        \robot{0}{.2cm}{gray}
        \robot{0}{.4cm}{gray}
        \robot{0}{.6cm}{gray}
        \robot{3}{0cm}{gray}
        \robot{3}{0.2cm}{gray}
        \robot{3}{0.4cm}{gray}
        \robot{3}{.6cm}{gray}
      \end{scope}
    \end{tikzpicture}
  \end{center}
%\end{overlayarea}
%\begin{overlayarea}{1\linewidth}{1cm}
%    {~}
%  \end{overlayarea}

\vfill
\end{slide}


\begin{slide}  
  \myheader[\hfill mise en œuvre]{Preuves d'impossibilité}

\vfill

%  \begin{overlayarea}{\linewidth}{4cm}
  \begin{center}
    \begin{tikzpicture}[scale=1.6]
      \node(dummy) at (-2,-1.5) {};
      \node(dummy) at (+3,+3) {};
      \begin{scope}[>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{3}{0cm}{gentil}
        \robot{3}{0.2cm}{gentil}
        \robot{3}{0.4cm}{gentil}
        \robot{3}{0.6cm}{gentil}
        \robot{0}{0cm}{gentil}
        \robot{0}{.2cm}{gentil}
        \robot{0}{.4cm}{gentil}
        \robot{0}{.6cm}{gentil}
        \node(col11) at (0,0) {};
        \node(col12) at (0,1cm) {};
        \node(col122) at (0,0.83cm) {};
        \node(col21) at (3,0) {};
        \node(col22) at (0,1.56cm) {\rule{0pt}{2pt}};
        \node(col31) at (1.7,0) {};
        \node(col32) at (1.7,0.75cm) {};
        \draw[->,color=red,inner sep=2pt,line width=3pt] (col122) 
        to [out=65,in=110] node [above] {\emphr{?}} (col32) ;
      \end{scope}
      \node(eq) at (5.5,0) {\Huge$\equiv$};
      \begin{scope}[xshift=4cm,>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{0}{0cm}{gray}
        \robot{0}{.2cm}{gray}
        \robot{0}{.4cm}{gray}
        \robot{0}{.6cm}{gray}
        \robot{3}{0cm}{gray}
        \robot{3}{0.2cm}{gray}
        \robot{3}{0.4cm}{gray}
        \robot{3}{.6cm}{gray}
      \end{scope}
    \end{tikzpicture}
  \end{center}
%\end{overlayarea}
%\begin{overlayarea}{1\linewidth}{1cm}
%    {~}
%  \end{overlayarea}

\vfill
\end{slide}

\begin{slide}  
  \myheader[\hfill mise en œuvre]{Preuves d'impossibilité}

\vfill

%  \begin{overlayarea}{\linewidth}{4cm}
  \begin{center}
    \begin{tikzpicture}[scale=1.6]
      \node(dummy) at (-2,-1.5) {};
      \node(dummy) at (+3,+3) {};
      \begin{scope}[>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{3}{0cm}{gentil}
        \robot{3}{0.2cm}{gentil}
        \robot{3}{0.4cm}{gentil}
        \robot{3}{0.6cm}{gentil}
        \robot{0}{0cm}{gentil}
        \robot{0}{.2cm}{gentil}
        \robot{0}{.4cm}{gentil}
        \robot{0}{.6cm}{gentil}
        \node(col11) at (0,0) {};
        \node(col12) at (0,1cm) {};
        \node(col122) at (0,0.83cm) {};
        \node(col21) at (3,0) {};
        \node(col22) at (3,1cm) {};
        \node(col31) at (1.7,0) {};
        \node(col32) at (1.7,0.75cm) {};
        \node[draw=red,inner sep=10pt,thick,ellipse,fit=(col11) (col12)] {};
        % \draw[->,color=red,inner sep=2pt,line width=3pt] (col122) 
        % to [out=65,in=110] node [above] {\emphr{?}} (col32) ;
      \end{scope}
      \node(eq) at (5.5,0) {\Huge$\equiv$};
      \begin{scope}[xshift=4cm,>=stealth,inner sep=5pt, node distance=1cm,thick,line width=.8pt]
        \draw [color=black] (-1.5,-5pt) -- (4.6,-5pt);
        \robot{0}{0cm}{gray}
        \robot{0}{.2cm}{gray}
        \robot{0}{.4cm}{gray}
        \robot{0}{.6cm}{gray}
        \robot{3}{0cm}{gray}
        \robot{3}{0.2cm}{gray}
        \robot{3}{0.4cm}{gray}
        \robot{3}{.6cm}{gray}
      \end{scope}
    \end{tikzpicture}
  \end{center}
%\end{overlayarea}
%\begin{overlayarea}{1\linewidth}{1cm}
%    {~}
%  \end{overlayarea}

\vfill
\end{slide}




